Toward the Engineering of Virtuous Machines

While various traditions under the 'virtue ethics' umbrella have been studied extensively and advocated by ethicists, it has not been clear that there exists a version of virtue ethics rigorous enough to be a target for machine ethics (which we take to include the engineering of an ethical sensibility in a machine or robot itself, not only the study of ethics in the humans who might create artificial agents). We begin to address this by presenting an embryonic formalization of a key part of any virtue-ethics theory: namely, the learning of virtue by a focus on exemplars of moral virtue. Our work is based in part on a computational formal logic previously used to formally model other ethical theories and principles therein, and to implement these models in artificial agents.

==> evaluation.tex <==

How well does the formal system above adhere to Alfano's Conditions?
We outline a quick evaluation below (with our explanations emphasized):

The goal in this paper is to evaluate how well $\mathcal{V}^f_z$
adheres to the conditions laid out by Alfano in
\citelow{alfano2013identifying}. Alfano lays out a series of
conditions that he considers to be the core of virtue ethics. The
conditions are laid below:

%% NAVEEN: The footnote seems to be incomplete.  Can you check it?
%% //S
 



\begin{footnotesize}
\begin{mdframed}[linecolor=white, frametitle= Alfano's Hard Core of Virtue Ethics (from
  \citelow{alfano2013identifying}), frametitlebackgroundcolor=gray!15,
  backgroundcolor=gray!06, roundcorner=8pt]

\begin{enumerate}[(1)]
\item \textbf{acquirability} It is possible for a non-virtuous person
  to acquire some of the virtues. \emph{Learning is central to \Vf.}
\item  \textbf{stability} If someone possesses a virtue at time $t_1$,
  then \emph{ceteris paribus} she will possess that virtue at a later time
  $t_2$.  \emph{Once a trait is learnt, it cannot be lost.}
\item \textbf{consistency}   If someone possesses a virtue sensitive to
  reason $r$, then \emph{ceteris paribus} she will respond to $r$ in most
  contexts. \emph{Definition of a trait.}
\item \textbf{access} It is possible to determine what the virtues
  are. \emph{By examing when the emotion of admiration is consistently
    triggered, one can isolated virtuous traits.}

\item \textbf{normativity} \emph{Ceteris paribus}, it is better to
  possess a virtue than not, and better to possess more virtues than
  fewer. \emph{Admiration is triggered only for actions that are beneficial.}
\item \textbf{real saints}  There is a non-negligible cohort of saints
  in the human population. \emph{Not relevant for machine ethics.}
\item \textbf{explanatory power}  If someone possesses a virtue, then reference to that
virtue will sometimes help to explain her behavior. \emph{Definition
  of a trait.} 
\item \textbf{predictive power} If someone possesses a high-fidelity
  virtue, then reference to that virtue will enable nearly certain
  predictions of her behavior; if someone possesses a low fidelity
  virtue, then reference to that virtue will enable weak predictions
  of her behavior. \emph{Definition
  of a trait.} 
\item \textbf{egalitarianism} Almost anyone can reliably act in
  accordance with virtue. \emph{Definition of a traits and learning of
    traits.}
\end{enumerate}
\end{mdframed}
\end{footnotesize}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> objections.tex <==
 

 \noindent  \textbf{Objection 1} \emph{While the presented approach checks out in terms of formal logic, naturally, it cannot quite escape the anthropocentric nature of virtues on a meta-ethical level.}

 \noindent \textbf{Response} We agree with this statement. Virtue
 ethics talks about virtues of \emph{persons}, and because of this a
 non-person centric version of virtue ethics might not be
 possible. This is not an issue with our approach but with virtue
 ethics in general.

\noindent  \textbf{Objection 2} \emph{Why were Alfano's conditions chosen?}

\noindent \textbf{Response} Our goal is not to formalize or espouse
one ethical theory. Our goal is to build mathematical and
computational tools for implementing a wide range of ethical theories.
For example, given an ethical theory $\mathcal{E}$, this task is made
easier when there is a rigorous but still informal version
$\mathcal{E}_r$ that we can formalize as $\mathcal{E}^f_r$. On the
other hand, we need to have independent ways of evaluating whether
formalizations $\mathcal{E}^f_r$ capture $\mathcal{E}$. Alfano's
conditions are the most rigorous set of \emph{empirically grounded} claims that we have
come across for virtue ethics that serves the evaluation purpose .

\noindent \textbf{Objection 3} \emph{I don't see how the statement `if someone possesses a
  virtue sensitive to reason r, then ceteris paribus she will respond
  to r in most contexts' is captured by the definition of a trait.}

\noindent\textbf{Response} By the way a trait is defined, actions
performed by an agent in situations that triggers a trait $\tau$ will
be instances of an action type $\alpha$, these instances will be
largely similar (as they are instantiated from \emph{one} action type).

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> questions.tex <==

This formalization lets us address the following two
questions: ($\mathbf{Q_1}$): When can we say an agent is virtuous?,
and ($\mathbf{Q_2}$): How can an agent become virtuous?





%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> ve_overview.tex <==



\section{Virtue Ethics:  Overview and Exemplarism}
\label{sect:ve_over_exemplarism}


\subsection{\VE\ is Somewhat Unfamiliar to Folks}
%% Explain that VE is a bit unfamiliar, in context
  The core concepts of consequentialist ethical theories (i.e.\ of
  members of \CE), at least certainly in the particular such theory
  known as \textit{utilitarianism}, are doubtless at minimum
  relatively familiar to most of our readers.  For instance, most in
  our audience will know that utilitarianism's core tenet is that
  actions are obligatory just in case they have the consequence of
  maximizing happiness, and are forbidden exactly when they fail to so
  maximize.  A parallel state-of-affairs holds for at least basic
  knowledge of deontological ethical theories (= family \DE): most
  readers have for instance some familiarity with Kant's moral system
  in family \DE, and specifically with his famous ``categorical
  imperative,'' which, paraphrasing, says that, unconditionally, one
  must always act in such a way that this behavior could be
  universalized.\footnote{This imperative is first set out in --- as
    it's known in abbreviation --- \textit{Groundwork}; see
    \cite{practical_philosophy_with_groundwork}.  It's generally
    thought by ethicists, and this may be convenient for machine/AI
    ethics, that Kant had in mind essentially a decision procedure to
    follow in the attempt to behave in an ethically correct manner.
    For a lucid and laconic overview of this point, see
    \cite{sep_kant_moral_philosophy}; and
    cf.\ \cite{powers_kantian_machine}.} In addition, generally people
  are familiar with the core tenet of divine-command ethical theories
  (i.e.\ of members of \DCE), which is (approximately) that actions
  are obligatory for humans if and only if God commands that these
  actions be performed (a particular member of \DE is specified in
  \cite{quinn_divine_command}).  However, in our experience the
  epistemic situation is radically different when it comes to the
  family of ethical theories \textit{virtue ethics} (= \VE).  For
  while it's true that generally educated people can be assumed to be
  acquainted with the concept of virtue, and with many things long
  deemed to be virtues (e.g.\ bravery), an understanding of virtue
  ethics at the level of ethical \emph{theory} cannot be assumed.  We
  therefore now provide a rapid (and admittedly cursory) synopsis of
  \VE, by drawing from \cite{vallor_ve_book}, and to some degree from
  \cite{intelligent_virtue}.  It will be seen that \VE\ makes central
  use of examplars, and of learning and development that revolves
  around them.  Hence we shall arrive at a convenient entry point for
  our AI work devoted to trying to design and build a virtuous robot.



\subsection{Vallor's Affirmation of Exemplars and Learning}
%% Extraction from Vallor's book:
  Obviously we cannot in the span of the space we have at hand do full
  justice to the book-length treatment of \VE\ that is
  \cite{vallor_ve_book}.  But we can quickly establish that our
  technical work, in its focus on the cultivation of virtue for a
  machine via a focus on exemplars, is not merely based on a single,
  idiosyncratic member of \VE, and on one peripheral aspect of this
  member.  On the contrary, study of the work of Vallor and other
  scholars concerned with a characterization of the family
  \VE\ confirms that our exploitation specifically of Zagzebski's
  \cite{zagzebski2010exemplarist} focus, from the standpoint of the
  field of ethics itself, a worthy point of entry for AI researchers.

  To begin, Vallor, drawing on and slighly adapting Van Norden's
  \cite{van_norden_ve_consequentialism} sets out a quartet of
  commonalities that at least seem to be true of all members of \VE,
  and the second one is: ``A conception of moral virtues as cultivated
  states of character, manifested by those exemplary persons who have
  come closest to achieving the highest human good'' (\P 5, \S
  2.2).\footnote{In her book, Vallor gives her own more detailed and
    technologically relevant list of seven core elements that can be
    viewed as common to all members of \VE\ (or two what she refers to
    as ``traditions'' within virtue ethics).  We do not have the space
    to discuss this list, and show that it fits nicely with our
    technical work's emphasis on exemplars and learning therefrom.}
  But given our specific efforts toward engineering a virtuous
  machine, it is important to note that Vallor specifically informs us
  about the key concepts of exemplars in the particular members of the
  \VE\ family; to pick just one of many available places, she writes:

    \begin{small}
    \begin{quote}
      Buddhism's resonances with other classical virtue traditions do
      not end here.  As with the central role granted by Confucian and
      Aristotelian ethics to `exemplary persons' (the \textit{junzi}
      and \textit{phronimoi} respectively), \textit{bodhisattbas}
      (persons actively seeking enlightenment) generally receive
      direction to or assitance on the path of self-cultivation from
      the community of exemplary persons to which they have access.
      In Buddhism this is the monastic community and lay members of
      the \textit{Sangha} $\ldots$ [\P 5, \S 2.1.3,
        \cite{vallor_ve_book}]
    \end{quote}
    \end{small}



\subsection{Annas's Book Fits Too}
%
%% What about Annas's book?  Here we go:
%
  We said above that we would also draw, albeit briefly, from a second
  treatment of \VE, viz.\ \cite{intelligent_virtue}, in order to pave
  the way into our AI-specific, exemplar-based work.  About this
  second treatment we report only that it is one based squarely on a
  ``range of development'' (\P 3, \S Right Action in Ch.\ 3), where
  the agent (a human in her case) gradually develops into a truly
  virtuous person, beginning with unreflective adoption of direct
  instruction, through a final phase in which ``actions are based on
  understanding gained through experience and reflection'' (ibid.).
  Moreover, Annas explicitly welcomes the analogy between an agent's
  becoming virtuous, and an agent's becoming, say, an excellent
  tennis-player or pianist.  The idea behind the simularity is that
  ``two things are united: the \emph{need to learn} and the
  \emph{drive to aspire} (emphasis hers; \P 4 Ch.\ 3).  In addition,
  following Aristotle on \VE\ (e.g.\ see
  \cite{aristotle_nicomachean_ethics} 1103), no one can become a
  master tennis-player or pianist without, specifically, playing
  tennis/the piano with an eye to how the great exemplars work their
  mastery in these two domains.






\subsection{Transition \P}
%% Transition paragraph:
  In order to now turn to specific AI work devoted to engineering a
  virtuous robot, we move from completed consideration of the general
  foundation of \VE, and its now-confirmed essential use of moral
  exemplars, to a specific use of such exemplars that appears ripe for
  mechanization.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

